Multi-Sender Persuasion: A Computational Perspective

We consider the multi-sender persuasion problem: multiple players with informational advantage signal to convince a single self-interested actor to take certain actions. This problem generalizes the seminal Bayesian Persuasion framework and is ubiquitous in computational economics, multi-agent learning, and multi-objective machine learning. The core solution concept here is the Nash equilibrium of senders' signaling policies. Theoretically, we prove that finding an equilibrium in general is PPAD-Hard; in fact, even computing a sender's best response is NP-Hard. Given these intrinsic difficulties, we turn to finding local Nash equilibria. We propose a novel differentiable neural network to approximate this game's non-linear and discontinuous utilities. Complementing this with the extra-gradient algorithm, we discover local equilibria that Pareto dominates full-revelation equilibria and those found by existing neural networks. Broadly, our theoretical and empirical contributions are of interest to a large class of economic problems.

==> macros.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{note}[theorem]{Note}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheoremstyle{nonindented}{1ex}{1ex}{}{}{\bfseries}{.}{.5em}{}
\newtheoremstyle{indented}{1ex}{1ex}{\itshape\addtolength{\leftskip}{0.6cm}\addtolength{\rightskip}{0.6cm}}{}{\bfseries}{.}{.5em}{}
\theoremstyle{nonindented}
%\newtheorem{domain}{Game Domain}
\theoremstyle{indented}
%\newtheorem{question}{Question}[section]
%\newtheorem*{direction*}{Research Direction}
%\newtheorem*{conjecture*}{Conjecture}
\theoremstyle{plain}



\newenvironment{proofof}[1]{\begin{proof}[Proof of #1]}{\end{proof}}
\newenvironment{proofsketch}{\begin{proof}[Proof Sketch]}{\end{proof}}
\newenvironment{proofsketchof}[1]{\begin{proof}[Proof Sketch of #1]}{\end{proof}}

\newenvironment{alg}{\begin{algorithm}\begin{onehalfspace}\begin{algorithmic}[1]}{\end{algorithmic}\end{onehalfspace}\end{algorithm}} 

\newcommand{\mult}{\times}
\newcommand{\cross}{\times}
\newcommand{\by}{\times}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\card}[1]{\left| #1 \right|}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}
\newcommand{\bigunion}{\bigcup}
\newcommand{\bigintersect}{\bigcap}
\newcommand{\sm}{\setminus}
\newcommand{\floor}[1]{\lfloor {#1} \rfloor}
\newcommand{\ceil}[1]{\lceil {#1} \rceil}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}
\newcommand{\iid}{i.i.d.\ }

\newcommand{\lt}{\left}
\newcommand{\rt}{\right}


\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}

%Operators: These operators are such that a subscript appears below
%in \[ \] math mode, and to the bottom right in regular $ $ math mode

%regular version
\def\pr{\qopname\relax n{Pr}}
\def\ex{\qopname\relax n{E}}
\def\min{\qopname\relax n{min}}
\def\max{\qopname\relax n{max}}
\def\argmin{\qopname\relax n{argmin}}
\def\argmax{\qopname\relax n{argmax}}
\def\avg{\qopname\relax n{avg}}


%bold version
\def\Pr{\qopname\relax n{\mathbf{Pr}}}
\def\Ex{\qopname\relax n{\mathbf{E}}}
\def\supp{\qopname\relax n{\mathbf{supp}}}
\def\Min{\qopname\relax n{\mathbf{min}}}
\def\Max{\qopname\relax n{\mathbf{max}}}
\def\Argmin{\qopname\relax n{\mathbf{argmin}}}
\def\Argmax{\qopname\relax n{\mathbf{argmax}}}
\def\Avg{\qopname\relax n{\mathbf{avg}}}
\def\vol{\qopname\relax n{\mathbf{vol}}}
\def\aff{\qopname\relax n{\mathbf{aff}}}
\def\conv{\qopname\relax n{\mathbf{convexhull}}}
\def\hull{\qopname\relax n{\mathbf{hull}}}

\newcommand{\expect}[2][]{\ex_{#1} [#2]}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\RRp}{\RR_+}
\newcommand{\RRpp}{\RR_{++}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}

\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\def\I{\mathcal{I}}
\def\J{\mathcal{J}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\P{\mathcal{P}}
\def\R{\mathcal{R}}
\def\S{\mathcal{S}}
\def\O{\mathcal{O}}
\def\T{\mathcal{T}}
\def\V{\mathcal{V}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}

\def\eps{\epsilon}
\def\sse{\subseteq}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\Bmat}[1]{\begin{Bmatrix} #1 \end{Bmatrix}}
\newcommand{\vmat}[1]{\begin{vmatrix} #1 \end{vmatrix}}
\newcommand{\Vmat}[1]{\begin{Vmatrix} #1 \end{Vmatrix}}
\newcommand{\mat}[1]{\pmat{#1}}
\newcommand{\grad}{\bigtriangledown}
\newcommand{\one}{{\bf 1}}
\newcommand{\zero}{{\bf 0}}


\newcommand{\hl}[1]{{\bf \color{red}#1}}
\newcommand{\todo}[1]{{\hl{To do: #1}}}
\newcommand{\todof}[1]{{\hl{ (Todo\footnote{\hl{\bf  To do: #1}})}}  }
\newcommand{\noi}{\noindent}
\newcommand{\prob}[1]{\vspace{.2in} \noindent {\bf Problem #1.}\\}
\newcommand{\subprob}[1]{ \vspace{.2in} \noindent {\bf #1.}\\}


%Plain eps or pdf figure. Use IPE to embed tex in it.
\newcommand{\fig}[2][1.0]{
  \begin{center}
    \includegraphics[scale=#1]{#2}
  \end{center}}
%Combined PS/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined ps/latex" option
\newcommand{\figpst}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pstex_t}}
  \end{center}}
%Combined PDF/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined pdf/latex" option
\newcommand{\figpdft}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pdf_t}}
  \end{center}}



%Algorithmic Environment stuff
\newcommand{\INPUT}{\item[\textbf{Input:}]}
\newcommand{\OUTPUT}{\item[\textbf{Output:}]}
\newcommand{\PARAMETER}{\item[\textbf{Parameter:}]}


%LP environment stuff
\newcommand{\mini}[1]{\mbox{minimize} & {#1} &\\}
\newcommand{\maxi}[1]{\mbox{maximize} & {#1 } & \\}
\newcommand{\maximin}[1]{\mbox{max min} & {#1 } & \\}
\newcommand{\find}[1]{\mbox{find} & {#1 } & \\}
\newcommand{\st}{\mbox{subject to} }
\newcommand{\con}[1]{&#1 & \\}
\newcommand{\qcon}[2]{&#1, & \mbox{for } #2.  \\}
\newenvironment{lp}{\begin{equation}  \begin{array}{lll}}{\end{array}\end{equation}}
\newenvironment{lp*}{\begin{equation*}  \begin{array}{lll}}{\end{array}\end{equation*}}




%% MISC





==> text/2-Related.tex <==
\subsection{Additional Related Works}
Closest to ours are works on Bayesian persuasion with multiple senders: e.g., \cite{gentzkow_bayesian_2017, li2021sequential, ravindran_competing_2022}. 
\citet{gentzkow_bayesian_2017} study a model where the senders can correlate their signals and \citet{li2021sequential} study a model with sequential senders who choose signaling policies after observing previous senders'.
These two models are different from ours which assumes that, conditioning on the realized state, the senders send signals to the receiver \emph{independently} and \emph{simultaneously}.  We think our model is more natural and better captures the motivating examples in our Introduction, and is also technically more challenging. 

\citet{ravindran_competing_2022} also study Bayesian persuasion games with multiple independent and simultaneous senders, but assuming zero-sum utility for the senders.  They show that, under some conditions, a Nash equilibrium is full revelation (every sender fully reveals the state to the receiver) and this is the \emph{only} equilibrium.
Many multi-sender persuasion games, however, do not satisfy zero-sum utility. 
An important question left from their work is thus: in multi-sender persuasion games with general utilities, do other types of equilibria than full-revelation exist?  We provide a positive answer to this question. 

Lastly, while all the multi-sender Bayesian persuasion works mentioned above characterize Nash equilibria from an economic perspective, we also take a computational approach, showing that finding non-full-revelation equilibrium in multi-sender Bayesian persuasion is computationally hard. 

For other variants of the standard single-sender Bayesian persuasion problem \cite{kamenica2011bayesian}, one can refer to \cite{dughmi_2017_survey}, \cite{kamenica2019bayesian}, and \cite{bergemann_information_2019} for overviews.

% Bayesian persuasion where senders and receivers have different priors: \cite{alonso_bayesian_2016}.

% Bayesian persuasion where the receiver has private types: \cite{kolotilin_persuasion_2017, dughmi_algorithmic_2017}


==> text/4-Analysis.tex <==
\section{Theoretical Equilibrium Analysis}

\begin{lemma}[Best Response]\label{lemma:best_response}
    The best response for sender $j$, given a set of schemes for other senders $\bpi_{-j}$, can be expressed as a linear program with $|\Sig||\Omega|$ variables and $|\mathcal{A}|^2 + |\Omega|$ constraints.
\end{lemma}

\begin{theorem}[Existence]\label{thm:existence}
    Any multi-sender persuasion game with a subjective signal interpretation $\alpha$ admits an $\alpha$-NE.
\end{theorem}


\begin{theorem}[Full-revelation equilibrium]\label{thm:characterization}
    Suppose $|S| \geq |\A|^{\tfrac{1}{n-1}}$ and for every state $\omega$, there is a unique optimal action for the receiver. Then there always exists a subjective fixed interpretation $\alpha$ such that an $\alpha$-NE that fully reveals the state exists.
\end{theorem}
\sh{The condition of for every state $\omega$, there is a unique optimal action for the receiver is pretty simple and standard. could just keep this assumption in the model.}

\begin{corollary}
    $\alpha$-NE need not be unique for an arbitrary instance.
\end{corollary}

\begin{theorem}[PPAD-hardness]\label{thm:PPAD}
    Finding $\alpha$-NE in multi-sender persuasion games is PPAD-hard, even if there are only $|\Omega|=2$ states, $n=2$ senders, and $|\A|=4$ actions for the receiver (while the signal space $|\Sig|$ is large.) 
\end{theorem}
\sh{Can we extend the PPAD result to show hardness in the number of senders for fixed number of signals?}
\tl{This is tricky.  When there are multiple senders, encoding the signal interpretation already takes $\log( |A|^{|S|^n} ) = |S|^n \log |A|$ bits, which is exponential in $n$.  So even if the computational complexity is exponential in $n$, it can still be polynomial in the ``input size''. }

==> text/old_results.tex <==
\section{Missing Proofs}

\subsection{Proof of Lemma~\ref{lemma:best_response}}
\begin{proof}
Consider the following linear program for influencer $i$ that solves for their signaling scheme $\pi_i(s_i|\omega)$, given a fixed scheme for other influencer $\bpi_{-i}(\bs_{i}|\omega)$:

\begin{gather}
      \text{maximize}~~ \sum_{\bs \in \Sig} \sum_{\omega \in \Omega} {\pi_i(s|\omega)\bm{\pi_{-i}}(\bm{s}_{-i} | \omega)\mu_0(\omega)u_i(\alpha(\bm{s}), \omega)} \text{\quad \quad \quad \quad \quad \, } \\
      \text{subject to:} \sum_{\omega}\pi_i(s_i|\omega)\bm{\pi_{-i}}(\bm s_{-i}|\omega)\mu_0(\omega)\left[u_r(\alpha(\bm{s}), \omega) - u_r(a_{j}, \omega)\right] \geq 0 \, , \, \forall \bm{s} \in \Sig^n, \forall a_j \ne \alpha(\bm{s}) \\
      \sum_{s \in \Sig}{\pi_i(s | \omega)} = 1 \, , \, \forall \omega \in \Omega
\end{gather}

Note for the incentive compatibility constraint, we require the following holds for the posterior induced by any joint signal $\bs$: $\sum_{\omega}{P(\omega|\bs)\left[u_r(\alpha(\bm{s}), \omega) - u_r(a_{j}, \omega)\right]}$. By Bayes rule, $P(\omega|\bs) = \frac{\bpi(\bs|\omega)\mu_0(\omega)}{P(\bs)}$ and since $P(\bs)$ is constant for the whole sum, we can multiply both sides by $P(\bs)$ and arrive at the constraint in the above LP. This ensures when the agent computes her posterior belief upon receiving any joint signal $\bs$ with respect to the joint signaling scheme $\bpi = (\pi_j, \bpi_{-j})$, the actors interpretation for that signal, $\alpha(\bs)$ is indeed utility maximizing. Combined with the objective, this linear program maximizes for the ex-ante utility for influencer $j$ amongst all possible IC signaling schemes.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:existence}}
\begin{proof}
The best response for any influencer $i$, depends on the policy of others: $\text{br}_i(\bm{\pi}_{-i})$, which we defined formally in lemma \ref{lemma:best_response}. Note that this may be empty if the linear program is infeasible and need not be unique if it is. Now consider the joint best response correspondence $\text{br}(\bm{\pi}) = [\text{br}_1(\bm{\pi}_{-1}) , \dots, \text{br}_n(\bm{\pi}_{-n})]$ which defines the best response for every influencer under a joint signalling scheme $\bm{\pi}$. For a surjective scheme $\alpha$, let $\Theta$ denote the set of all joint signals $\bpi$ which are IC w.r.t.~$\alpha$.

We first show that $\Theta$ is non-empty. Since $\alpha$ is surjective it must be the case that $|\Sig|^n \geq |\mathcal{A}|$. Next, for each state $\omega$, let $a_\omega$ denote the best agent action for that state, and consider any joint signal $\bs_{\omega} \in \alpha^{-1}(a_\omega)$. Then it is clear that the joint signaling scheme $\bpi(\bs_{\omega}|\omega)$ is incentive compatible for the agent. Next, the IC constraints each influencer best response satisfies implies that if $\bpi \in \Theta$, any $\bpi' \in \text{br}(\bpi)$ must also satisfy IC constraints with respect to $\alpha$, and thus $\bpi' \in \Theta$. Lastly, we show that the set $\Theta$ is convex. Let $\bm{\pi}_1$ and $\bm{\pi}_2$ be two joint signals that belong to $\Theta$. Since this implies that both joint signaling schemes are IC w.r.t.~$\alpha$, the following always holds for any $\bm{s}, a_j$, and $\lambda \in [0,1]$: 
    \begin{gather}\label{eq:equi_exist_ic_1}
        \sum_{\omega}{\lambda \bm{\pi}_1(\bm{s}|\omega)\mu_0(\omega)[u_r(\alpha(\bm{s}), \omega) - u_r(a_j, \omega)]} \geq 0 \\
        \sum_{\omega}{(1-\lambda) \bm{\pi}_2(\bm{s}|\omega)\mu_0(\omega)[U_r(\alpha(\bm{s}), \omega) - U_r(a_j, \omega)]} \geq 0 
    \end{gather}
By adding these two equations, we can state the following for any $\bm{s}, a_j$:
    \begin{align}\label{equation:convex_ic}
        \sum_{\omega}{[\lambda\bm{\pi}_1(\bm{s}|\omega)+(1-\lambda) \bm{\pi}_2(\bm{s}|\omega)]\mu_0(\omega)[U_r(\alpha(\bm{s}), \omega) - U_r(a_j, \omega)]} \geq 0
    \end{align}
Clearly, $\lambda \bpi_1 + (1-\lambda)\bpi_2$ is a valid signaling scheme that also satisfies the IC constraints. Putting all this together, we have that the set of jointly feasible strategies is a non-empty convex set $\Theta$, and the joint best response is a correspondence mapping from $\Theta$ to $2^{\Theta}$, where $2^{\Theta}$ is a set whose elements are all members of $\Theta$.

Next, for notational ease we define the ex-ante utility for influencer $i$ as a function of the scheme $\bpi$ as $\tilde{u}_i(\pi_i, \bpi_{-i}) = \sum_{\bs, \omega}{\pi(s_i|\omega)\bm{\pi}_{-i}(\bm{s}_{-i} | \omega)\mu_0(\omega)u_i(\alpha(\bm{s}), \omega)}$. Observe that this function is linear in $\pi_i$, for any fixed $\bpi_{-i}$. We next follow a technique from \citet{rosen1965existence} and for any two joint signaling schemes $\bpi^1, \bpi^2 \in \Theta$, consider the function: $\rho(\bpi^1, \bpi^2) = \sum_{i=1}^{n}{\tilde{u}_i(\pi^2_i, \bpi^1_{-i})}$. We briefly note that while the joint signaling scheme $(\pi^2_i, \bpi^1_{-i})$ may not actually be IC (and thus not belong to $\Theta$), $\tilde{u}$ is still well defined for this. Note that $\rho(\bpi^1, \bpi^2)$ is continuous in both $\bpi^1, \bpi^2$, and linear (and thus concave) in $\bpi^2$ for any fixed $\bpi^1$. Next, for any $\bpi^1$, define the correspondence $\zeta(\bpi^1) = \{\bpi^2 | \rho(\bpi^1, \bpi^2) = \max_{\bpi' \in \Theta}{\rho(\bpi^1, \bpi')}\}$, and note that $\zeta$ is an upper hemi-continious correspondence due to the continuity and linearity properties of $\rho$. Further, since $\zeta$ is a correspondence from an element in a convex set $\Theta$ to a subset within $\Theta$, we can apply Kakutani fixed point theorem to assert that there exists a $\bpi^* \in \Theta$ such that $\bpi^* \in \zeta(\bpi^*)$. It is evident that $\bpi^*$ is a PNE. Belonging to $\Theta$ already implies it satisfies IC constraints, and note that if for some influencer $i$, there was a unilateral profitable deviation $\pi'_i$, then $\tilde{u}_i(\pi'_i, \bpi^*_{-i}) > \tilde{u}_i(\pi^*_i, \bpi^*_{-i})$, which implies that for $\bpi' = (\pi_i',, \bpi^*_{-i})$, $\rho(\bpi^*, \bpi') \geq \rho(\bpi^*, \bpi^*)$ which implies $\bpi^*$ cannot the fixed point of correspondence $\zeta$. 
\end{proof}

